Towards Multimodal In-Context Learning for Vision & Language Models

State-of-the-art Vision-Language Models (VLMs) ground the vision and the language modality primarily via projecting the vision tokens from the encoder to language-like tokens, which are directly fed to the Large Language Model (LLM) decoder. While these models have shown unprecedented performance in many downstream zero-shot tasks (eg image captioning, question answers, etc), still little emphasis has been put on transferring one of the core LLM capability of In-Context Learning (ICL). ICL is the ability of a model to reason about a downstream task with a few examples demonstrations embedded in the prompt. In this work, through extensive evaluations, we find that the state-of-the-art VLMs somewhat lack the ability to follow ICL instructions. In particular, we discover that even models that underwent large-scale mixed modality pre-training and were implicitly guided to make use of interleaved image and text information (intended to consume helpful context from multiple images) under-perform when prompted with few-shot demonstrations (in an ICL way), likely due to their lack of direct ICL instruction tuning. To enhance the ICL abilities of the present VLM, we propose a simple yet surprisingly effective multi-turn curriculum-based learning methodology with effective data mixes, leading up to a significant 21.03% (and 11.3% on average) ICL performance boost over the strongest VLM baselines and a variety of ICL benchmarks. Furthermore, we also contribute new benchmarks for ICL evaluation in VLMs and discuss their advantages over the prior art.

==> tables/MME_average.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lccccc}
\toprule
 &\textbf{Total Cognition} & \textbf{Total Perception}  \\ 
 \hline
{Llava1.5} & 295.36 & 1531  \\ 
{Ours} & 301.43 & 1520.15 \\ 
\bottomrule
\end{tabular}
\caption{MME Performance total scores in Cognition and perception categories for llava1.5 and Our Model. Please see supplementary for detailed results.}
\label{tab:average_MME_scores}
\end{table}

==> tables/MME_cognition.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lccccc}
\toprule
 &\textbf{Total} & \shortstack{Commonsense\\Reasoning} & \shortstack{Numerical\\Calculation} & \shortstack{Text\\Translation} & \shortstack{Code\\Reasoning} \\ \hline
{Llava1.5} & 295.36 & 127.86 & 42.5 & 77.5 & 47.5 \\ 
{Ours} & 301.43 & 136.43 & 50 & 55 & 60 \\ 
\bottomrule
\end{tabular}
\caption{MME Performance scores in Cognition category for llava1.5 and Our Model}
\label{tab:cognition_scores}
\end{table}

==> tables/MME_perception.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
 & \textbf{Total} & {Existence} & {Count} & {Position} & {Color} & {Posters} \\ 
 \hline
{Llava1.5} & 1531 & 185 & 155 & 133.33 & 170 & 160.54 \\ 
{Ours} & 1520.15 & 195 & 140 & 138.33 & 185 & 147.96 \\ 
\bottomrule
\toprule
 & {Celebrity} & {Scene} & {Landmark} & {Artwork} & {OCR} \\ 
 \hline
{Llava1.5} & 152.94 & 161.25 & 167.31 & 117.75 & 125 \\ 
{Ours} & 157.65 & 161.25 & 153.21 & 131.75 & 110 \\ 
\end{tabular}

\caption{MME Performance scores in Perception category for llava1.5 and Our Model}
\label{tab:perception_scores}
\end{table}

==> tables/data_format_mixes.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
\shortstack{Mix\\ID} &\shortstack{Attributes} & \shortstack{Relations} & \shortstack{Categories} & {Instances} & \shortstack{AVG\\Accuracy} \\ \hline
% SEED mc 
1  & 0.00\% & 0.00\% & 0.00\% & 100.00\% & 56.56 \\ 
% SEED mc + LLava oq 
2  & 0.00\% & 0.00\% & 0.00\% & 100.00\% & 65.41 \\ 
% SEED mc + LLava oq + VL(0) op + VL(0) mc 
3  & 66.67\% & 	0.00\% & 	0.00\% & 	33.33\%  & 66.35 \\ 
% SEED mc + LLava oq + VL(0) op + VL cap 
4 & 75.00\% &	12.50\% &	0.00\% &	12.50\%  & 68.44 \\ 
% SEED mc + LLava oq + VL op + VL mc + VL cap 
5 & 45.45\% &	15.15\% &	36.36\% &	3.03\%  & 69.33 \\ \bottomrule
\end{tabular}
\caption{Shared semantic concept (between ICL shots in the same any-shot instruction) mixing ablation.}
    \label{tab:instruction_format_mixes}
\end{table}


==> tables/format_mix_ablation.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lccc|c}
\toprule
\shortstack{Mix\\ID} & \shortstack{Open\\Questions} & \shortstack{Multiple\\Choice} & {Captioning} & \shortstack{Avg\\Accuracy} \\
\hline
% SEED mc 
1 & 0.00\% & 100.00\% & 0.00\% & 56.57 \\
% SEED mc +LLava oq 
2 & 0.00\% & 100.00\% & 0.00\% & 65.41 \\
% SEED mc +LLava oq + VL(0) op 
3 & 50.00\% & 50.00\% & 0.00\% & 66.54 \\
% SEED mc +LLava oq + VL cap + VL op 
4 & 65.00\% & 5.00\% & 30.00\% & 69.14 \\
% SEED mc +LLava oq + VL op +VL mc +VL cap 
5 & 39.39\% & 42.42\% & 18.18\% & 69.33 \\
\bottomrule
\end{tabular}
\caption{Instruction format mixes effect on Model performance.}
\label{tab:instruction_format_mixes}
\end{table}

==> tables/main_table.tex <==
% \definecolor{positive}{rgb}{0,0.6,0}

\begin{table}
\centering
\small 
\caption{Comparison of models across various metrics.}
\label{tab:model_comparison}
\begin{tabular}{lcccccc}
\toprule
Model & SEED 23 & Unseen & Ins Count & MC VL & QA VL & Cap VLs \\
\midrule
IDEFICS 9B & 45 & 27 & 28 & 63.77 & 10.00 &  2.37 \\
OpenFlamingo & 25 & 24.8 & 18.25 & 45.00 &0.77 &0.41\\
Llava1.6 13B & 40.8 & 59 & 49 & 88.00 & 19.48 & 2.27 \\
EMU2 & - & 44.15 & 30.9 & 67.60 & 12.00 & 2.25 \\    
Llava-1.5 13B & 44.17 & 61 & 60 & 33.00 & 1.56 & 5.62 \\
% llava-1.5-our & 42.5 & 59 & 55 & 58.88 & 69.39 & 71.75 \\
\hline
Ours 13B & 49.16\gcol{+4.16} & 62.2\gcol{+3.20} & 65.3\gcol{+16.30} & 95.37\gcol{+7.37} & 24.5\gcol{+5.02} & 23.4\gcol{+21.03} \\
\bottomrule
\toprule
Model & Food & Cars & Dogs & CUB & Flowers & \textbf{AVG} \\
\midrule
IDEFICS 9B & 65.94 & 77.3 & 50.93 &  62  & 55.29 & 44.33 \\
OpenFlamingo &24.29&	53.93 & 21.64 & 12.75 & 5.15 & 21.09 \\
Llava1.6 13B & 89.15 & 84.7 & 72.39 & 67.9 & 65.58 & 58.02 \\
EMU2 & 59.92 & 55.42 & 50.27 & 53.56 & 52.76 & 42.88 \\
Llava-1.5 13B& 87.19 & 57.3 & 33 & 58.24 & 58.6 & 47.50 \\
% llava-1.5-our & 94.54 & 82.79 & 88 & 19.91 & 4.67 & 58.77 \\
\hline
Ours 13B & 98.3 \gcol{+9.15} & 97.9\gcol{+13.20} & 84.1\gcol{+11.71} & 82.3\gcol{+14.40} & 80.1\gcol{+14.52} & 69.33 \gcol{+11.31} \\
\bottomrule


\end{tabular}
\end{table}

% 4.16	3.2	16.3	11.71	14.4	14.52	9.15	13.2	7.37417034	5.016159704	21.03186641	11.30572805


==> tables/model_ablation.tex <==
\begin{table}
\centering
\small 
\caption{Comparison of models across various metrics.}
\label{tab:model_comparison}
\begin{tabular}{lcccccc}
\toprule
Model & SEED 23 & Unseen & Ins Count & AVG Dogs & AVG CUB & AVG Flowers \\
\midrule
Llava-1.5 & 44.17 & 61 & 60 & 58.24 & 55.8 & 58.6 \\
% llava-1.5-our & 42.5 & 59 & 55 & 58.88 & 69.39 & 71.75 \\
SEED mc & 12.5 & 61 & 61 & 75.24 & 78.75 & 64.37 \\
SEED mc + Llava oq & 40.83 & 63 & 66 & 83.38 & 82.43 & 74.66 \\
+ VL(0) op & 40.83 & 63 & 70 & 84.00 & 82.93 & 77.18 \\
+ VL(0) op + mc & 42.5 & 64 & 66 & 82.67 & 80.47 & 79.64 \\
+ VL op + mc & 39.17 & 62 & 69 & 73.36&	75.74&	69.27\\
% + VL(0) mc+op+VL cap & 46.6 & 63.4 & 65.3 & 83.62 & 84.58 & 79.44 \\
+ VL op + cap & 46.67 & 61.29 & 63.75 & 85.64 & 91.37 & 79.60 \\
+ VL op + mc + cap & 49.16 & 62.2 & 65.3 & 84.1 & 82.3 & 80.1 \\
\bottomrule
\toprule
Model & Avg Food & Avg Cars & MC VL & QA VL & Cap VL & AVG \\
\midrule
Llava-1.5 & 87.19 & 57.3 & 33 & 1.56 & 5.62 & 47.50 \\
% llava-1.5-our & 94.54 & 82.79 & 88 & 19.91 & 4.67 & 58.77 \\
SEED mc & 93.02 & 91.12 & 85.12 & 0.14 & 0 & 56.57 \\
SEED mc + Llava oq & 96.97 & 94.68 & 90.94 & 20.55 & 6.09 & 65.41 \\
+ VL(0) op & 98.25 & 96.90 & 92.97 & 19.90 & 5.94 & 66.54 \\
+ VL(0) op + mc & 98.50 & 96.95 & 93.31 & 19.95 & 5.93 & 66.36 \\
+ VL op + mc &	93.17&	91.55& 96.28 & 31.03 & 7 & 64.32 \\
% + VL cap & 98.25 & 96.87 & 90.77 & 20.50 & 23.57 & 68.45 \\
+ VL op + cap & 98.50 & 97.99 & 89.70 & 21.42 & 24.64 & 69.14 \\
+ VL op + mc + cap & 98.3 & 97.9 & 95.37 & 24.5 & 23.4 & 69.33 \\
\bottomrule


\end{tabular}
\end{table}

==> tables/one_vs_many_shots_VL.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lccc}
\hline
& MC VL & QA VL & Cap VL \\
\hline
Two-shot & 95.37 & 24.5 & 23.4 \\
One-shot & 87.9 & 12.9 & 0 \\
Zero-shot & 87.4 & 12.5 & 0 \\
\hline
\end{tabular}
\caption{many vs one shot with best model}
\label{tab:one_shot}
\end{table}

